On the evolution of the Anisotropic Scaling of Magnetohydrodynamic Turbulence in the Inner Heliosphere

We analyze a merged Parker Solar Probe ($PSP$) and Solar Orbiter ($SO$) dataset covering heliocentric distances $13 \ R_{\odot} \lesssim R \lesssim 220$ $R_{\odot}$ to investigate the radial evolution of power and spectral-index anisotropy in the wavevector space of solar wind turbulence. Our results show that anisotropic signatures of turbulence display a distinct radial evolution when fast, $V_{sw} \geq ~ 400 ~km ~s^{-1}$, and slow, $V_{sw} \leq ~ 400 ~km ~s^{-1}$, wind streams are considered. The anisotropic properties of slow wind in Earth orbit are consistent with a ``critically balanced'' cascade, but both spectral-index anisotropy and power anisotropy diminish with decreasing heliographic distance. Fast streams are observed to roughly retain their near-Sun anisotropic properties, with the observed spectral index and power anisotropies being more consistent with a ``dynamically aligned'' type of cascade, though the lack of extended fast-wind intervals makes it difficult to accurately measure the anisotropic scaling. A high-resolution analysis during the first perihelion of PSP confirms the presence of two sub-ranges within the inertial range, which may be associated with the transition from weak to strong turbulence. The transition occurs at $\kappa d_{i} \approx 6 \times 10^{-2}$, and signifies a shift from -5/3 to -2 and -3/2 to -1.57 scaling in parallel and perpendicular spectra, respectively. Our results provide strong observational constraints for anisotropic theories of MHD turbulence in the solar wind.

==> notes.tex <==
These include (i) The $\it{variance \ anisotropy}$, i.e., the magnitudes of
the fluctuations in directions

parallel and perpendicular to the
mean magnetic field, and spectral anisotropy is determined with
respect to the direction of k


the unequal distribution of power in the spectra of the turbulent fluctuations with wavenumbers parallel ($\boldsymbol{\kappa}_{||}$) and perpendicular ($\boldsymbol{\kappa}_{\perp}$) to the mean magnetic field  \citep{belcher_large-amplitude_1971, zhao}
(ii)  correlation  lengths  parallel  toB0were  found  to  bemuch  larger  than  those  in  directions  perpendicular  toB0
spectral anisotropy

Anisotropy in the solar wind has been examined in terms of (i) 
the inertial range spectral indices of



 ($\tau_{nl}(\boldsymbol{|k|})$) 
 

Additionally, in-situ measuremanets of anisotropy in the solar wind reported puzzling results and also raised concerns that need to be adressed, e.g., disparities between velocity field and magnetic field anisotropy


The synergy of the Parker Solar Probe ($PSP$)  \citep{fox_solar_2016} and Solar Orbiter ($SO$) missions has furthered our understanding of the properties of the solar wind inner heliosphere \citep[see e.g.,,][]{kasper_PSP_alfven, 2022arXiv220807932B}).


   % F_{ii}(f_{sc}^{m}, ~ \theta_{BV}) = \frac{4 \pi}{C \omega_{0} N} \sum_{ \{ n: ~  \theta_{j-1} \leq \theta_{BV} \leq \theta_{j} \}}|\omega_{i} (s_{m}, t_{n})|^{2},
    % F_{ii}(f_{sc}, ~ \theta_{BV}) = \frac{4 \pi}{C \omega_{0} N} \sum_{n=0}^{N-1}|\omega_{i} (s_{m}, t_{n}, \theta_{BV})|^{2},
    

    


% , for which $f\approx 1/(1.033 s)$, $f$ is the Fourier frequency, and $\ell_{m} = \ell_{0}2^{m \cdot\delta m}$, $m = 0,...., M$, where, $M = \delta m ^{-1}log_{2}(N \delta t/\ell_{0})$ and $\delta m$ defines the spacing between consecutive scales.
    
    
    


% In the following we examine the evolution of the spectral indices with heliocentric distance by considering  overlapping intervals of duration $d = 24$hrs sampled by PSP and SolO throught the inner heliosphere (see, Section \ref{subsec:Data_processing}). A visual inspection of the selected intervals was conducted, and those containing coronal mass ejections and solar wind speeds exceeding $400 ~kms^{-1}$ were discarded. After estimating the power spectral density for each interval, $E(\kappa^{*},~ \theta_{BV})$, the local spectral index, $\alpha_{B}(\kappa^{\ast})$, was 
% obtained by taking a sliding window of size $w = ~10$ in $\kappa^{\ast}$, over the spectra and calculating the best-fit linear gradient in log-log space over this window. Subsequently, an average local spectral index was estimated for intervals falling within each of six heliocentric-radii bins. Despite the fact that the original spectra, as well as the local spectral indices, were calculated at identical frequencies depending on the duration of the interval and the sampling frequency, the normalization process results in a shift along the vertical axis that is irregular. For this reason, the entire range of $\kappa^{\ast}$ was divided into 100 bins, and the mean was calculated for all $\alpha_{B}(\kappa^{\ast})$ values falling in each bin, \citep{Nemecek_2021}. To ensure statistical significance of our results, each bin was required to have a minimum number of 100 data points.  The resulting $\alpha_{B}(\kappa^{\ast})$  as a function of heliocentric distance, in blue and red for parallel and perpendicular spectra, respectively, is illustrated in  Figure \ref{fig:PSD_evol}. Error bars are also shown, indicating the mean error of the power-law fit. It is important to point out that in this study we focus our attention on MHD scales, $\kappa^{\ast} \leq 3 \times 10^{-1} ~ [d_{i}^{-1}]$. This is because as the spacecraft moves farther away from the sun, the amplitude of the fluctuations at kinetic scales, is close to the noise-floor of the magnetometer. This leads to an artificial steepening of PSD caused by instrumental noise \citep{phdthesis}. The effect is particularly significant for $\alpha_{B}(\kappa^{\ast})$  parallel, since most of the power in the solar wind is associated with wavevectors polarized perpendicular to the mean magnetic field, and thus the parallel PSD systematically obtains lower values at MHD and kinetic scales.
% Considering the results, it is apparent that the inertial range spectral anisotropy diminishes as the heliocentric distance decreases. Within 0.1 au, only minor differences may be observed in
% $\alpha_{B}(\kappa^{\ast})$ for parallel and perpendicular fluctuations. 






As the solar wind expands into the interplanetary medium the inertial range for both parallel and perpendicular spectra extends to progressively larger scales, while at the same time steepening in a scale dependent fashion. At heliocentric distances between 0.1-0.2 au, the -2 scaling appears in the parallel PSD extending over a limited range of scales just before the transition region, while the perpendicular spectrum steepens $\alpha_{B}^{\perp}\approx -5/3$ and $\alpha_{B}^{  ||}\approx -2$ appears, though more clear in the high resolution data of E1, (see Figure \ref{fig:SCaM:E1_PSD}. The steepened region becomes more pronounced in the 0.2-0.3 au bin, especially for $E_{\delta B_{||}}$. Within $\approx0.3-0.4 au$, see also Figure 4 in \citep{sioulas_turb_22_no1}, the perpendicular scaling is consistent with the IK scaling, $\alpha_{B} =-3/2$. Beyond this point the spectrum steepens towards $\alpha_{B} =-5/3$, even at the largest scales, just before the energy injection range a $-3/2$ scaling can be observed at all distances .

As the solar wind expands in the inner heliosphere, the inertial range for both parallel and perpendicular spectra extends to progressively larger scales, while also steepening in a scale-dependent fashion. At distances between 0.1-0.2 au, the scaling exponents are qualitatively similar to the ones shown in Figure \ref{fig:SCaM:E1_PSD}. Sub-range $R^{1}$ is characterized by a scaling index of $-5/3$ and $-3/2$ in the parallel and perpendicular directions, respectively, while a steepened sub-range appears just before the transition region. The steepened region, $R^2$, is not as clearly defined as in Figure \ref{fig:SCaM:E1_PSD}, which may be due to the fact that a large number of intervals with different plasma parameters have been averaged to obtain the final curve.

In the 0.2-0.3au bin, the steepened region becomes more prominent, particularly for parallel fluctuations. A similar scaling  is observed in the parallel direction between $0.3-0.4 au$, while the perpendicular PSD is observed to gradually steepen from an IK scaling, $\alpha_{B} =-3/2$, towards a K41 scaling with increasing distance. Observations and critical balance predictions show good agreement at distances greater than about 0.5 au, with inertial range scaling exponents of -2 and -5/3, respectively, for parallel and perpendicular PSDs.


